InfAnFace: Bridging the infant-adult domain gap in facial landmark estimation in the wild

We lay the groundwork for research in the algorithmic comprehension of infant faces, in anticipation of applications from healthcare to psychology, especially in the early prediction of developmental disorders. Specifically, we introduce the first-ever dataset of infant faces annotated with facial landmark coordinates and pose attributes, demonstrate the inadequacies of existing facial landmark estimation algorithms in the infant domain, and train new state-of-the-art models that significantly improve upon those algorithms using domain adaptation techniques. We touch on the closely related task of facial detection for infants, and also on a challenging case study of infrared baby monitor images gathered by our lab as part of in-field research into the aforementioned developmental issues.

==> response.tex <==
\newcommand{\response}{
\clearpage
%\onecolumn
\newcommand{\beginresponse}{%
        \setcounter{table}{0}
        \setcounter{equation}{0}
        \renewcommand{\theequation}{R\arabic{equation}}
        \setcounter{section}{0}
        \renewcommand{\thetable}{R\arabic{table}}%
        \setcounter{figure}{0}
        \renewcommand{\thefigure}{R\arabic{figure}}%
}

\section{Response to Reviewers}

We thank the Editor and the Reviewers for their thoughtful comments. We start with some general contextual remarks and a description of new work done for this revision, and then turn to individual responses.

\subsection{General comments and additions to revised manuscript}

We see the computer vision study of infant facial landmarks, which we initiate in this paper, as an important step towards the application of machine learning to infant and child developmental healthcare. Our technical contribution includes the creation of the first dataset of infant faces with landmark annotations (i.e., InfAnFace), the use of our dataset to characterize and analyze the poor performance of existing state-of-the-art facial landmark estimation models on infant faces, and the use of domain adaptation and data augmentation techniques---informed by our analysis and our dataset and comprehensively tuned with validation testing---to develop new models that perform well on infant faces. One highlight from our results is that our model achieves a 2.50\% failure rate on infant faces compared to 22.50\% from existing state-of-the-art, approaching the 1.17\% of state-of-the-art performance on comparable adult faces. We believe this serves as a strong baseline for the field.

For this revision, we have made the following additions in response to Reviewer comments:
\begin{enumerate}
    \item We trained a number of new models and reported their performance metrics in \secref{infant-landmarking-models}. In the original submission, we implemented a number of HRNet variations and also tested with the pretrained 3FabRec model. For this revision, we implemented similar variations for the 3FabRec model (3FabRec-FT, 3FabRec-JT, 3FabRec-R90, and 3FabRec-R90JT), nearly doubling the number of new models considered. The updated results demonstrate the effectiveness of our general methods with a new backbone model, buttressing our original conclusions. This code will also be made available at press time.
    \item We added a brief discussion of why commonly used advanced domain adaptation methods based around adversarial domain discrimination, like DANN \cite{ganin_domain-adversarial_2016} and ADDA \cite{tzeng_adversarial_2017}, are not effective in our setting. Namely, adversarial domain discrimination methods target classification tasks, but for a task involving regression like landmark estimation, the covariate shift condition means that such methods will actually decrease performance in the target domain, as discussed in \cite{kivinen_domain_2011} and especially \cite{de_mathelin_adversarial_2021}. (We also confirmed this in practise with some informal tests with HRNet augmented with the DANN framework.) Thus, we believe that our models are already quite strong in the spectrum of models obtainable by general domain adaptation techniques which apply in our setting.
    \item We added a new visualization in \figref{mean-face-errors} of the landmark estimation error on a per-landmark basis.
    \item We have made numerous presentation additions and improvements, many in response to issues raised by Reviewers, as detailed below.
    \item We have moved some less critical material from the original paper to a new Supplementary Section (\secref{supplementary}). The main paper remains complete as a stand-alone work.
\end{enumerate}


\subsection{Reviewer 4, Review 1701}

[Reviewer comments reproduced in plain text. \textbf{Our responses in bold.}]

This paper presents multi-pronged efforts to initiate and foster an ecosystem of infant facial landmark estimation research. The author proposed a new database as a primary contribution.

The paper in the actual conditions is not ready to be published. The method contribution is not clear. I can identify some problems such as face detection, alignment and pose estimation. According to the space available to the paper, the author must focus on only one of these problems deeper.

\textbf{We have made major modifications in response to these critiques, as outlined below.}

The author proposed the HRNet-R90JT  and HRNet-R90FT; however, no explanation is given about the configuration of the network.

\textbf{We have added short descriptions of the underlying HRNet and 3FabRec networks and a schematic diagram of the HRNet structure (\figref{hrnet}).  We also have clarified how we modified the HRNet training regime with targeted domain adaptation and data augmentation to produce our HRNet-R90JT and HRNet-R90FT versions.}

The face detection and application sections are missing because of the superficial discussion.

\textbf{Face detection is a part of the full facial landmark estimation pipeline (see our next answer), so we discuss it in our paper. However, since our experiments show that existing SOTA face detection is excellent on infant faces, we felt that the overall pipeline was sufficiently complete. The application to nighttime baby monitor footage is a difficult challenge problem, akin to the most challenging adult facial datasets, so in this paper we focus on establishing the baseline results on more standard infant data (which already includes some challenging poses).}

The face-detection stage is working very fine in this kind of image. Why do I need to improve the landmark? Please discuss. 

\textbf{Face detection only yields a rectangular box indicating where the face is, whereas facial landmark estimation yields the locations and orientations of the eyes, nose, mouth, cheeks, etc., providing much more fine-grained facial information for potential applications. We have clarified this in the main text.}

The T-SNE distribution does not help too much. It may be an analysis of the number of landmarks points most interesting to see. 

\textbf{We have modified the t-SNE visualization in \figref{t-sne} so that it more clearly illustrates the adult vs. infant domain gap, and within infants, the common vs. challenging poses. We follow an industry standard Multi-PIE landmark configuration which fixes the number of landmarks at 68. We have added a visualization in \figref{mean-face-errors} of the prediction error on a per-landmark basis, which is indeed instructive.} 

Landmark detection uses the centre of the pupil or eyes to align images. According to the photos, please indicate it is necessary to use 68 landmarks for infants? 

\textbf{One of our error metrics is normalized by the interocular distance, defined as the distance between the outer corners of the eyes, which are included as part of the 68 landmarks in the Multi-PIE configuration that we adopt. These 68 landmarks do not include the centers of the eyes but they can be estimated by averaging other eye landmarks. Some datasets use around 20 landmarks, and a few use 98 landmarks, but 68 is common thanks in part to the prolific 300-W dataset. This higher granularity in infant facial landmark detection hopefully enables the early detection of oral-motor disorders in infancy, that otherwise may manifest more severely in older age if not diagnosed/treated on time.}

Please. Table 4 include or clarify units. Regarding the same table, the AUC of 48 or 55, Must be considered good?

\textbf{We have added the information that both failure rate (FR) and area under the curve (AUC) are out of 100 (so they can also be interpreted as percentages), and that lower FR and higher AUC are better. AUC is indeed hard to interpret but it can perhaps be considered a slightly more stable alternative to FR. NME, FR, and AUC are frequently reported in facial landmark estimation.}

In summary, I suggest that the authors focus on the landmark detection problem and analyses the results considering landmark numbers. Face detection and application are also relevant, but they do not have much space for this discussion in a six-page paper.

\textbf{We have reduced the space taken by the discussion of face detection, and we have increased our analysis of facial landmark estimation by implementing new training regimes for the 3FabRec model and reporting their performance metrics, as outlined in our general comments above. We thank Reviewer 4 for their many thoughtful comments and suggestions.}


\subsection{Reviewer 7, Review 2295}

The main contribution of the paper is the introduction of the InfAnFace dataset. 

The authors described the process they went through to gather the dataset. 

The authors illustrate the gap between infant faces and adult faces by comparing the stats of the locations in the new dataset and some other well-known datasets. 

The authors used HRNet to base their improvements by applying simple and different augmentation and fine-tuning procedures. 

The authors evaluated the non-infant-based architectures and the updated versions both qualitatively and quantitatively. 

The authors finally tested their models on specialized test cases on 15 infants. However, the results are not very accurate yet.

My comments are that

1. I like the paper writing. The authors made it easy to read and follow.

2. Table I is not correct. The sums don't match the 210 and 200 totals.

\textbf{The attributes tabulated in that table overlap and thus the values do not need to sum to 210 and 200, but we agree that the table layout strongly suggests that they should, so we have changed the layout to clear up this confusion.}

3. The results show improvements over the baselines. However, the contribution and ideas are very basic to add augmentation and fine-tuning. 

\textbf{For our revised submission we have added some further experimental results and additional context for our contributions, which are also summarized in our general comments above.}

4. My overall recommendation is to accept the paper.

\textbf{We thank Reviewer 7 for their comments and clear synopsis of our work.}


\section{Reviewer 8, Review 2297}

Interesting paper.

Font size in Fig. 5 \& 6 needs to be enlarged.

\textbf{Thank you, we have increased the type size and clarity in these and other figures in the paper.}


\subsection{Reviewer 10, Review 2305}

This paper shows the facial landmark detection for infant face, which is quite important for recent applications including h-care, psychology or safety fields. The paper developed the dataset of infant faces annotated with facial landmark and poses, and trained the facial models. As the result, the accuracy of landmark detection improved and developped real-life application showcase.

Personally, I like this work regarding the development of infant-face landmark dataset -- which is quite valuable for the communicaty. However, the paper lack technical contribution regarding the algorithm. 

\textbf{We have added some further experimental results and additional context for our contributions in our revised submission, and these are also summarized in our general comments above. We offer our thanks to Reviewer 10 for their summary and assessment. }

}

